Data-dependent Initializations of Convolutional Neural Networks

Convolutional Neural Networks spread through computer vision like a wildfire, impacting almost all visual tasks imaginable. Despite this, few researchers dare to train their models from scratch. Most work builds on one of a handful of ImageNet pre-trained models, and fine-tunes or adapts these for specific tasks. This is in large part due to the difficulty of properly initializing these networks from scratch. A small miscalibration of the initial weights leads to vanishing or exploding gradients, as well as poor convergence properties. In this work we present a fast and simple data-dependent initialization procedure, that sets the weights of a network such that all units in the network train at roughly the same rate, avoiding vanishing or exploding gradients. Our initialization matches the current state-of-the-art unsupervised or self-supervised pre-training methods on standard computer vision tasks, such as image classification and object detection, while being roughly three orders of magnitude faster. When combined with pre-training methods, our initialization significantly outperforms prior work, narrowing the gap between supervised and unsupervised pre-training.

==> figures/scaling/mean_poster.tex <==
\begin{tikzpicture}[scale=0.7]
\begin{semilogyaxis}[
    legend cell align=left,
    height=0.9\textwidth,
    width=1.5\textwidth,
    title={},
    xlabel={},
%
    ylabel absolute, ylabel style={yshift=-1em},
    xmin=0, xmax=7,
    ymin=0, ymax=1000,
    ymajorgrids=true,
    legend pos=north east,
    legend columns=2,
    grid style=dashed,
    xtick={0, 1, 2, 3, 4, 5, 6, 7},
    xticklabels={\rotatebox{90}{conv1}, \rotatebox{90}{conv2}, \rotatebox{90}{conv3}, \rotatebox{90}{conv4}, \rotatebox{90}{conv5}, \rotatebox{90}{fc6}, \rotatebox{90}{fc7}, \rotatebox{90}{fc8}},
]

\addplot[color=ta3butter,ultra thick,solid] coordinates {(0,35.004200)(1,21.994300)(2,16.632500)(3,16.596000)(4,19.116000)(5,6.542880)(6,7.779460)(7,13.315900)}; \addlegendentry{Gaussian}
\addplot[color=ta3scarletred,ultra thick,dashed] coordinates {(0,7.145320)(1,4.395430)(2,3.510380)(3,3.616200)(4,6.232390)(5,6.694680)(6,11.193900)(7,12.313200)}; \addlegendentry{Gaussian (caffe)}
\addplot[color=ta3orange,ultra thick,dotted] coordinates {(0,10.951200)(1,10.876900)(2,10.853700)(3,10.800400)(4,10.888200)(5,10.757800)(6,10.113100)(7,10.634800)}; \addlegendentry{Gaussian (ours)}
\addplot[color=ta3chocolate,ultra thick,solid] coordinates {(0,12.083500)(1,11.369000)(2,10.795900)(3,10.722500)(4,10.400300)(5,10.893500)(6,9.075250)(7,12.080900)}; \addlegendentry{ImageNet}
%
%
\end{semilogyaxis}
\end{tikzpicture}



==> figures/scaling/variation_poster.tex <==
\begin{tikzpicture}[scale=0.7]
\begin{axis}[
    legend cell align=left,
    height=0.9\textwidth,
    width=1.5\textwidth,
    title={},
    xlabel={},
%
    ylabel absolute, ylabel style={yshift=-1.2em},
    xmin=0, xmax=7,
    ymin=0, ymax=30,
    legend pos=north east,
    legend columns=2,
    ymajorgrids=true,
    grid style=dashed,
    xtick={0, 1, 2, 3, 4, 5, 6, 7},
    xticklabels={\rotatebox{90}{conv1}, \rotatebox{90}{conv2}, \rotatebox{90}{conv3}, \rotatebox{90}{conv4}, \rotatebox{90}{conv5}, \rotatebox{90}{fc6}, \rotatebox{90}{fc7}, \rotatebox{90}{fc8}},
]

\addplot[color=ta3butter,ultra thick,solid] coordinates {(0,4.315340)(1,11.004800)(2,16.824000)(3,21.432200)(4,23.507200)(5,8.886080)(6,11.535800)(7,9.763660)};
\addplot[color=ta3scarletred,ultra thick,dashed] coordinates {(0,0.789607)(1,1.929000)(2,3.036550)(3,3.918840)(4,2.995850)(5,3.199120)(6,6.722430)(7,4.341240)};
\addplot[color=ta3orange,ultra thick,dotted] coordinates {(0,1.316830)(1,1.920170)(2,2.225150)(3,2.287510)(4,1.895550)(5,3.074480)(6,5.577490)(7,3.136590)};
\addplot[color=ta3chocolate,ultra thick,solid] coordinates {(0,4.097780)(1,5.550990)(2,5.258870)(3,5.064870)(4,5.421900)(5,14.205400)(6,16.603400)(7,6.576710)};
%
%
\end{axis}
\end{tikzpicture}


